Slow running of the Gradient Flow coupling from 200 MeV to 4 GeV in $N_{\rm f}=3$ QCD

Using a finite volume Gradient Flow (GF) renormalization scheme with Schr\"odinger Functional (SF) boundary conditions, we compute the non-perturbative running coupling in the range $2.2 \lesssim {\bar g}_\mathrm{GF}^2(L) \lesssim 13$. Careful continuum extrapolations turn out to be crucial to reach our high accuracy. The running of the coupling is always between one-loop and two-loop and very close to one-loop in the region of $200\,{\rm MeV} \lesssim \mu=1/L \lesssim 4\,{\rm GeV}$. While there is no convincing contact to two-loop running, we match non-perturbatively to the SF coupling with background field. In this case we know the $\mu$ dependence up to $\sim 100\,{\rm GeV}$ and can thus connect to the $\Lambda$-parameter.

==> Lswitch16.tex <==
\anote{Alberto?}{There should be something on the simulations 
giving the SF-coupling, in particular L=16 ! Patrick put something into the notes, 
but was it updated to the final status?}

==> app_ssf.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> hadronic.tex <==



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

